3DSAM-adapter: Holistic adaptation of SAM from 2D to 3D for promptable tumor segmentation

Despite that the segment anything model (SAM) achieved impressive results on general-purpose semantic segmentation with strong generalization ability on daily images, its demonstrated performance on medical image segmentation is less precise and not stable, especially when dealing with tumor segmentation tasks that involve objects of small sizes, irregular shapes, and low contrast. Notably, the original SAM architecture is designed for 2D natural images, therefore would not be able to extract the 3D spatial information from volumetric medical data effectively. In this paper, we propose a novel adaptation method for transferring SAM from 2D to 3D for promptable medical image segmentation. Through a holistically designed scheme for architecture modification, we transfer the SAM to support volumetric inputs while retaining the majority of its pre-trained parameters for reuse. The fine-tuning process is conducted in a parameter-efficient manner, wherein most of the pre-trained parameters remain frozen, and only a few lightweight spatial adapters are introduced and tuned. Regardless of the domain gap between natural and medical data and the disparity in the spatial arrangement between 2D and 3D, the transformer trained on natural images can effectively capture the spatial patterns present in volumetric medical images with only lightweight adaptations. We conduct experiments on four open-source tumor segmentation datasets, and with a single click prompt, our model can outperform domain state-of-the-art medical image segmentation models on 3 out of 4 tasks, specifically by 8.25%, 29.87%, and 10.11% for kidney tumor, pancreas tumor, colon cancer segmentation, and achieve similar performance for liver tumor segmentation. We also compare our adaptation method with existing popular adapters, and observed significant performance improvement on most datasets.

==> sections/Experiments.tex <==

\section{Experiments}
\subsection{Setup}
\noindent\textbf{Datasets.} We make our experiments focus on tumor segmentation, as this is the most challenging task for both medical imaging communities and the original SAM. To this end, we collect two public datasets for volumetric tumor segmentation, which include 1) Kidney Tumor Segmentation challenge 2021 dataset (\kits)~\cite{heller2020state} and 2) Pancreas Segmentation task of 2018 MICCAI Medical Segmentation Decathlon challenge dataset (\msd)~\cite{antonelli2022medical}. We employ 300 and 281 abdominal CT scans respectively. The original dataset includes both organ and tumor segmentation labels while we are only using tumor labels for training and testing. The datasets are randomly split into 70\%, 10\%, and 20\% for training, validation, and testing. 
More details can be found in the appendix.

\noindent\textbf{Implementation Details.} We implement our method and benchmark baselines in PyTorch and MONAI. We are using SAM-B for all the experiments and comparisons. The model is trained with batch size 1 on an NVIDIA A40 GPU, using AdamW~\cite{loshchilov2017decoupled} optimizer with a linear scheduler for 200 epochs. We set the initial learning rate of $1e^{-4}$, momentum of 0.9 and weight decay of $1e^{-5}$. We preprocess the data to have isotropic spacings of $1mm$. For data augmentation, we perform random rotation, flip, zoom, and shift intensity. We also randomly sample foreground/background patches at a ratio of 1:1 during training. The complete training details are available in the appendix. Overall, we evaluate the performance of our method via comparisons with current SOTA volumetric segmentation and fine-tuning approaches. The Dice coefficient (Dice) and Normalized Surface Dice (NSD) are used as evaluation metrics.

\subsection{Comparison with State-of-the-Art}

\begin{figure}[!tp]
    \centering
    \includegraphics[width=1\linewidth]{figures/vis.pdf}
    \caption{Qualitative visualizations of the proposed method and baseline approaches on kidney and pancreas tumor segmentation tasks.}
    \label{fig:vis}
\end{figure}

\begin{table}[t]
\footnotesize
\centering
\renewcommand\arraystretch{1}
    \caption{Comparison with classical medical imaging segmentation methods on kidney tumor segmentation and pancreas tumor segmentation. Dice score and normalized surface dice (NSD) are reported.}
\begin{center}
\label{tab:sota}
\begin{tabular}{l|cc|cc|c}
\toprule
\multirow{2}{*}{Methods\rule{0pt}{2.4ex}}&\multicolumn{2}{c|}{Kidney Tumor}&\multicolumn{2}{c|}{Pancreas Tumor} &\multirow{2}{*}{\#Tuned Params\rule{0pt}{2.4ex}}\\ [0.2ex]
 \cline{2-5}
  &Dice~$\uparrow$ &NSD~$\uparrow$&Dice~$\uparrow$&NSD~$\uparrow$ \rule{0pt}{2.4ex}\\
\midrule
nnU-Net (Nat. Methods 2021)~\cite{isensee2021nnu}  &73.07& 77.47 &41.65& 62.54& 30.76M \\
TransBTS (MICCAI 2021)~\cite{wang2021transbts}&40.79&37.74& 31.90 & 41.62&32.33M\\
nnFormer (arXiv 2021)~\cite{zhou2021nnformer}&45.14&42.28&36.53& 53.97&149.49M\\
 %UNETR &&&9.92&&10.92&&&\\
 Swin-UNETR (CVPR 2022)~\cite{tang2022self} &65.54&72.04&40.57&60.05&62.19M\\
 UNETR++ (arXiv 2022)~\cite{shaker2022unetr++}&56.49&60.04&37.25&53.59&55.70M\\
 3D UX-Net (ICLR 2023)~\cite{lee20223d} &57.59&58.55&34.83&52.56&53.01M\\
 \midrule
SAM-B (1 pt/slice)~\cite{kirillov2023segany} &36.30&29.86&24.01&26.74&--\\
Ours (1 pt/volume) &\textbf{73.78}&\textbf{83.86}&\textbf{54.09}&\textbf{76.27}&25.46M\\
\midrule
SAM-B (3 pts/slice))~\cite{kirillov2023segany} &39.66&34.85&29.80&33.24&-- \\
Ours (3 pts/volume) &\textbf{74.91}&\textbf{84.35}&\textbf{54.92}&\textbf{77.57}&25.46M\\
\midrule
SAM-B (10 pts/slice))~\cite{kirillov2023segany} &40.07&34.96&30.55&32.91&--\\
Ours (10 pts/volume) &\textbf{75.95}&\textbf{84.92}&\textbf{57.47}&\textbf{79.62}&25.46M\\
\bottomrule
\end{tabular}
\end{center}
\end{table}



We extensively compare our model with the recent volumetric medical image segmentation state-of-the-art. As reported in Table~\ref{tab:sota}, we observe that the original SAM~\cite{kirillov2023segany} developed in natural images gets suboptimal performances in domain-specific tumor segmentation tasks, even with massive clicks as prompts. With the proposed effective and efficient adaptation, we obtain state-of-the-art accuracy with a single point only in the whole volume, outperforming the powerful medical image segmentation baselines such as nnU-Net~\cite{isensee2021nnu}. Distinct improvements can be specifically observed for pancreas tumors, which are always notorious for ambiguous boundaries, of 12.44\% in Dice against the prior state-of-the-art. Besides, we observe stable performance rising when feeding more points for prompting. Our model gets Dice of 75.95\% and 57.47\% in kidney tumor and pancreas tumor segmentation respectively with 10 points per volume (which is usually affordable in common clinical usage). Relevant evidence is also observed in Fig.~\ref{fig:vis}, where SAM usually fails to distinguish tumor borders and gives false positive predictions, whereas our adaptation demonstrates visually better tumor identification results in both tasks.

\subsection{Comparison with Existing Volumetric Adaptation}
We further compare our adaptation strategy with existing parameter-efficient adaptation methods and also with the model of full fin-tuning. To conduct a fair comparison and be more focused on whether adaptations help the model learn volumetric medical image features,  we remove the prompt encoder and only train the model with an image encoder followed by a lightweight decoder (STER-MLA~\cite{zheng2021rethinking}). So that the model will conduct automatic segmentation without prompt guidance. The performance can well reflect the presentation learning ability of the encoder. All the pre-trained weights are from SAM-B. For comparison methods designed for 2D adaptation, we encode the images in a slice-wise manner and then concatenate them to form a 3D feature map before plugging them into the decoder.

The results are given in Table~\ref{adaptation}, which shows our adaptation strategy outperforms all existing methods with a comparable number of tuned parameters. Our method excels the second-best method by 16.24\% on kidney tumor segmentation Dice and 4.22\% on pancreas tumor segmentation NSD. It even outperforms many classical segmentation methods with fewer tunable parameters and a vanilla mask decoder. Our method also outperforms full fine-tuning of SAM by 17.76\% on kidney tumor segmentation and 14.00\% on pancreas tumor segmentation with only less than 17\% tunable parameters. These results can well substantiate our hypothesis that parameters pre-trained on 2D images can be used to learn 3D spatial features with only minor modifications. And treating all dimensions equally is actually a better strategy than interpreting the depth dimension as a group in medical image segmentation, especially when the images have similar spacings in all dimensions.
\begin{table}[t]
\footnotesize
\centering
\renewcommand\arraystretch{1}
\caption{Comparison with existing parameter-efficient and full fine-tuning methods. We discard the prompt encoder and only tune the image encoder and mask decoder for fully automatic segmentation.}
\label{adaptation}
\begin{center}
\label{adaptation}
\begin{tabular}{l|cc|cc|c}
\toprule
\multirow{2}{*}{Methods\rule{0pt}{2.4ex}}&\multicolumn{2}{|c|}{Kidney Tumor}&\multicolumn{2}{|c|}{Pancreas Tumor} &\multirow{2}{*}{{\makecell[c]{\#Tuned Params \\(image encoder)}}\rule{0pt}{2.4ex}}\\ [0.2ex]
 \cline{2-5}
  &Dice~$\uparrow$ &NSD~$\uparrow$&Dice~$\uparrow$&NSD~$\uparrow$ \rule{0pt}{2.4ex}& \\
\midrule
 %Scratch &&&&&&&& \\
 Full fine-tuning &52.31&50.35&26.49&33.28&89.67M\\
 Adapter (ICML 2019)~\cite{houlsby2019parameter}&46.99&43.76&20.28&30.81&7.61M\\
 Pro-tuning (arXiv 2022)~\cite{nie2022pro}&50.73&50.81&18.93&30.45&7.17M\\
 ST-Adapter (NeurIPS 2022)~\cite{pan2022st}&47.30&45.61&\textbf{30.27}&43.53&7.15M\\
 %AdaptFormer (NeurIPS 2022)~\cite{NEURIPS2022_ee604e1b}&40.43&38.17&32.39&48.83&12.30M\\
 %AIM&&&&&&&&\\
 Med-tuning (arXiv 2023)~\cite{wang2023med}&44.73&40.28&22.87&30.02&11.10M\\
 \midrule
 Ours&\textbf{61.60}&\textbf{70.40}&30.20&\textbf{45.37}&15.21M\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\subsection{Ablation Studies}
We also conduct comprehensive ablation studies regarding the design of the prompt encoder and mask decoder. 
%For the prompt encoder, we compare the model performance between using positional encoding and the visual sampler as the embedding of the points. We also analyze how the model performance is sensitive to the location and accuracy of the point prompts. For the decoder, we compare the model performance with and without multi-layer aggregation. We also experiment on the effects of deep prompts, i.e. cross attention with prompt attention on middle layers. 
The experiments are conducted on the KiTS 21 dataset and for each trial, we only give one point as a prompt while each result is based on 10 random trials. 
\begin{wrapfigure}{r}{5cm}
\footnotesize
\centering
\renewcommand\arraystretch{1}
\caption{Comparison of models w/o deep prompts.}
\label{deepprompt}
\begin{center}
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{4}{c|}{Feature Level}&\multirow{2}{*}{Dice~$\uparrow$\rule{0pt}{2.6ex}}&\multirow{2}{*}{NSD~$\uparrow$\rule{0pt}{2.6ex}}\\ [0.2ex] 
 \cline{1-4}
 1&2&3&4&& \rule{0pt}{2.6ex}\\
\midrule
\checkmark&\checkmark&\checkmark&\checkmark&64.61&71.33\\
\checkmark&&&\checkmark&66.82&74.87\\
&\checkmark&&\checkmark&69.17&77.49\\
&&\checkmark&\checkmark&65.39&72.56\\
&&&\checkmark&\textbf{73.78}&\textbf{83.86}\\
\bottomrule
\end{tabular}
\end{center}
\end{wrapfigure}

\noindent \textbf{Positional encoding v.s. visual sampler.}
In order to prove visual sampler is actually a better way for prompt encoding compared with the original positional encoding method used in SAM in terms of volumetric segmentation, we fix the image encoder and mask decoder while only changing the prompt encoder. The results are shown in Fig.~\ref{fig:ablation}. Our proposed visual sampler algorithm outperforms the original positional encoding by 40.00\% for Dice. This is align with our claim that visual sampler work well when the size of tokens is large as it does not have over-smoothing issues.


\noindent \textbf{Position of the point prompts.}
 We analyze how the model performance is different when the point prompt is given at the center of the objects, at its adjacent regions, or at the margin We divide the ground truth tumor mask into three regions, the center region, the surrounding region, and the marginal region, as illustrated in Fig~\ref{fig:ablation}. For cases with multiple tumors, we are sampling from the one with the largest size. From the results, we find that the model is not very sensitive to the position of the point prompts. Giving prompt at different positions yield almost the same results.

%\noindent \textbf{Noisy point prompts.}
%Inspired by the experimental result above, we consider giving prompts automatically, i.e. sampling points from the predicted masks of other segmentation algorithms as prompts. Thus, SAM can serve as a refinement to enhance the performance of other medical image segmentation models. To this end, we use nnU-Net as a shallow segmentation model. The results~\ref{} show SAM can significantly improve the performance of nnU-Net. Sometimes nnU-Net gives very coarse segmentation, but SAM can still help correct its prediction.

\noindent \textbf{Effects of multi-layer aggregation.} To verify  our modification of the mask decoder actually brings performance gain, we compare it with the one without multi-layer aggregation. The result~\ref{fig:ablation} shows the model with multi-layer aggregation has 15.75\% higher Dice than its counterpart. This also aligns with common practice in medical imaging segmentation as local texture features are very important, especially for tumor segmentation which usually has tiny shapes and low contrast.

\noindent \textbf{Effects of deep prompts.} Since it is beneficial to include features from multiple levels of the image encoder, a natural idea comes that incorporating prompts at multiple levels might also improve performance. To this end, we conduct experiments to plug in the prompt encoder to other feature levels besides the final bottleneck levels. The results are shown in Table~\ref{deepprompt}. However, we find incorporating deep prompts brings no gain or even degenerates the performance. This can be left as a topic for further research to make prompts take effect at multiple feature levels. 
\begin{figure}[!tp]
    \centering
    \includegraphics[width=1\linewidth]{figures/ablation.pdf}
    \caption{Results on our ablation studies. (a) Performance v.s prompt. (b) Visual sampler v.s. positional encoding. (c) Effects of multi-layer aggregation.} 
    \label{fig:ablation}
\end{figure}
